HairWeaver: Few-Shot Photorealistic Hair Motion Synthesis with Sim-to-Real Guided Video Diffusion

We present HairWeaver, a diffusion-based pipeline that animates a single human image with realistic and expressive hair dynamics. While existing methods successfully control body pose, they lack specific control over hair, and as a result, fail to capture the intricate hair motions, resulting in stiff and unrealistic animations. HairWeaver overcomes this limitation using two specialized modules: a Motion-Context-LoRA to integrate motion conditions and a Style-Alignment-LoRA to preserve the subject's photoreal appearance across different data domains. These lightweight components are designed to guide a video diffusion backbone while maintaining its core generative capabilities. By training on a specialized dataset of dynamic human motion generated from a CG simulator, HairWeaver affords fine control over hair motion and ultimately learns to produce highly realistic hair that responds naturally to movement. Comprehensive evaluations demonstrate that our approach sets a new state of the art, producing lifelike human hair animations with dynamic details.

==> Tables/6_add_ablation.tex <==

\begin{table}
\centering
\vspace{-9pt}
\caption{Additional ablation study on CG test set. 
% UVW maps achieve the best performance across most metrics, while the Alpha-map variant consistently outperforms the Wan-VACE baseline.
} 
\label{tab:cg_test_ablation}
\vspace{-1pt}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{l|ccccc|ccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{5}{c|}{\textbf{Hair}} & \multicolumn{5}{c}{\textbf{Full Body}} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11}
& \textbf{SSIM$\uparrow$} & \textbf{PSNR$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{FID$\downarrow$} & \textbf{cd-FVD$\downarrow$} & \textbf{SSIM$\uparrow$} & \textbf{PSNR$\uparrow$} & \textbf{LPIPS$\downarrow$} & \textbf{FID$\downarrow$} & \textbf{cd-FVD$\downarrow$} \\
\midrule
Wan-VACE (UVW)             & \underline{0.9724} & 34.6198            & 0.0348             & 57.9023            & 463.2543            & 0.8514             & 26.4512            & 0.1547             & 51.3914            & 412.5809            \\
\ourmodel (Alpha)    & \underline{0.9693}             & \underline{36.7297} & \underline{0.0236} & \textbf{49.0856}   & \underline{436.9389} & \underline{0.8710} & \underline{26.9807} & \underline{0.1340} & \underline{46.1248} & \underline{410.2243} \\
\ourmodel (UVW) & \textbf{0.9794}    & \textbf{37.6347}    & \textbf{0.0233}    & \underline{50.5938} & \textbf{434.1582}    & \textbf{0.8948}    & \textbf{27.7903}    & \textbf{0.1127}    & \textbf{43.2786}    & \textbf{407.1929}    \\
\bottomrule
\end{tabular}
}
\vspace{-18pt}
\end{table}
